Phase diagram and superconductivity of Calcium Alanates under pressure

In this paper we present a first-principles study of the high-pressure superconducting phase diagram of calcium alanates (Ca-Al-H), based on ab-initio crystal structure prediction and anisotropic Migdal-Eliashberg Theory. Calcium alanates have been intensively studied at ambient pressure for their hydrogen-storage properties, but their high-pressure behavior is largely unknown. By performing a full scan of the ternary convex hull at several pressures between 0 and 300 GPa, we identify several new structural motifs, characterized by a high Al-H coordination, where Al--$d$ orbitals participate in the bonding. Among all new phases thus identified, we focus in particular on a phase with CaAlH$_7$ composition, which lies on the convex hull at 300 GPa, and remains dynamically stable down to 50 GPa, with a predicted superconducting T$_c$ of 82 K, which likely represents a new promising template to achieve increase chemical precompression in ternary hydrides. Our findings reveal important insights into the structure-property relationships of calcium alanates under high pressure, and highlight a possible strategy to achieve conventional superconductivity at low pressures.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}
